Importance Weight Estimation and Generalization in Domain Adaptation under Label Shift

We study generalization under labeled shift for categorical and general normed label spaces. We propose a series of methods to estimate the importance weights from labeled source to unlabeled target domain and provide confidence bounds for these estimators. We deploy these estimators and provide generalization bounds in the unlabeled target domain.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/0-Old_Abstract.tex <==
We study generalization under label shift in domain adaptation where the learner has access to labeled samples from the source domain but unlabeled samples from the target domain. Prior works deploy label classifiers and introduce various methods to estimate the importance weights from source to target domains. They use these estimates in importance weighted empirical risk minimization to learn classifiers. In this work, we theoretically compare the prior approaches, relax their strong assumptions, and generalize them from requiring label classifiers to general functions. This latter generalization improves the conditioning on the inverse operator of the induced inverse problems by allowing for broader exploitation of the spectrum of the forward operator.

The prior works in the study of label shifts are limited to categorical label spaces. In this work, we propose a series of methods to estimate the importance weight functions for arbitrary normed label spaces. We introduce a new operator learning approach between Hilbert spaces defined on labels (rather than covariates) and show that it induces a perturbed inverse problem of compact operators. We propose a novel approach to solve the inverse problem in the presence of perturbation. This analysis has its own independent interest since such problems commonly arise in partial differential equations and reinforcement learning. 

% For both categorical and general normed spaces, we provide concentration bounds for the proposed estimators. Using the existing generalization analysis based on Rademacher complexity, R\'enyi divergence, and MDFR lemma in \citet{azizzadenesheli2019regularized}, we show the generalization property of the importance weighted empirical risk minimization on the unseen target domain.

For both categorical and general normed spaces, we provide concentration bounds for the proposed estimators which we later use to provide generalization for importance weighted empirical risk minimization on the unseen target domain.

==> Sections/5_1_neural.tex <==
\section{Neural Operator}
In this section, we further study the general normed spaces of y

==> Sections/Acknowledgements.tex <==
\IEEEraisesectionheading{\section*{Acknowledgements}"
The authors would like to thank Nikola Kovachki, Zongyi Li, and Burigede Liu for their insightful comments. The authors also would like to thank reviewer two of ALT 2021 for their comment on the construction of the $\Hilbert$ spaces in this paper. 

==> Sections/Appx_var.tex <==
\section{$\varepsilon$-approximation of $\Hilbert$}\label{apx:var_approximate}



In the following, we assume that for any $\Prob,
\Qrob\in\measures$, and their corresponding importance weight $\impW$, there exist a function ${\impWv}\in \Hilbert$, an $\varepsilon$-approximation of $\impW$ in $\Hilbert$, i.e., $\|\impW-\impWv\|_{\L^2(\Prob)}\leq \varepsilon$. We latter set $\varepsilon$ to be on the order of concentration errors, i.e., $\varepsilon=\mathcal{O}(\frac{1}{\sqrt{n}}\wedge\frac{1}{\sqrt{m}})$. 

Note that, we could also directly assume $\impW\in \Hilbert$, however, due to the work of \citet{minh2010some,steinwart2006explicit}, there are trivial functions, e.g. constant functions, that are not in standard $\Hilbert$'s. Therefore, our $\varepsilon$-relaxation of such strong assumption, generalizes the applicability of the results in this paper. 

 





\begin{align*}
    q_u:=\V_u(\Qrob) = \int_{(\X\times\Y)} k_{u(x)}d\Qrob(x,y) &=\E_\Qrob[k_{u}] \stackrel{a.s.}{=} E_\Qrob[E_\Qrob[k_{u}|\F_\Y]] \stackrel{a.s.}{=} E_\Qrob[E_\Prob[k_{u}|\F_\Y]]\\
    &\stackrel{a.s.}{=} E_\Prob[\impW E_\Prob[k_{u}|\F_\Y]] \stackrel{a.s.}{=} E_\Prob[(\impW-\impWv+\impWv) E_\Prob[k_{u}|\F_\Y]]\\
    &\stackrel{a.s.}{=}E_\Prob[(\impW-\impWv) E_\Prob[k_{u}|\F_\Y]]\leq \varepsilon\kappa + E_\Prob[\impWv E_\Prob[k_{u}|\F_\Y]]\\
    &\stackrel{a.s.}{=}E_\Prob[(\impW-\impWv) E_\Prob[k_{u}|\F_\Y]]\varepsilon\kappa+ E_\Prob[\kernel_Y^u\langle \kernel_Y,\impWv\rangle]\\
    &\stackrel{a.s.}{=}=E_\Prob[(\impW-\impWv) E_\Prob[k_{u}|\F_\Y]]+\T_u\impWv
\end{align*}
Note that $\|E_\Prob[(\impW-\impWv) E_\Prob[k_{u}|\F_\Y]]\|_{\L(\Prob)}\leq\varepsilon\kappa$, therefore negligible for sufficiently small $\varepsilon$.
